Follow-Your-Click: Open-domain Regional Image Animation via Short Prompts

Despite recent advances in image-to-video generation, better controllability and local animation are less explored. Most existing image-to-video methods are not locally aware and tend to move the entire scene. However, human artists may need to control the movement of different objects or regions. Additionally, current I2V methods require users not only to describe the target motion but also to provide redundant detailed descriptions of frame contents. These two issues hinder the practical utilization of current I2V tools. In this paper, we propose a practical framework, named Follow-Your-Click, to achieve image animation with a simple user click (for specifying what to move) and a short motion prompt (for specifying how to move). Technically, we propose the first-frame masking strategy, which significantly improves the video generation quality, and a motion-augmented module equipped with a short motion prompt dataset to improve the short prompt following abilities of our model. To further control the motion speed, we propose flow-based motion magnitude control to control the speed of target movement more precisely. Our framework has simpler yet precise user control and better generation performance than previous methods. Extensive experiments compared with 7 baselines, including both commercial tools and research methods on 8 metrics, suggest the superiority of our approach. Project Page: https://follow-your-click.github.io/

==> all_subtex/details.tex <==
\begin{table}[!ht]
\setlength{\tabcolsep}{4pt}
\caption{Hyperparameters for our \emph{approach}.}
\centering
\resizebox*{!}{.95\textheight}{
\setlength{\tabcolsep}{5pt}
    \begin{tabular}{lc}
    \toprule
    \textbf{Hyperparameter} & \textbf{\emph{Follow-Your-Click}}   \\
    \midrule\midrule
    \textbf{Spatial Layers}  &  \\
    \textit{Architecture} \\
    LDM & \cmark  \\
    % Pretrained &\cmark \\
    $frames$ & 16 \\
    $z$-shape & $32 \times 32 \times 4$  \\
    Channels & 320 \\
    Depth & 2 \\
    Channel multiplier & 1,2,4,4\\
    Attention resolutions & 64,32,16\\
    Head channels & 64 \\
    Input channels & 8 \\
    Output channels & 4 \\
    \midrule
    \emph{OPM Conditioning} & \\
    Embedding dimension & 768 \\
    FPS sampling range & 1--16\\
    \midrule
    \emph{Concat Conditioning} & \\
    Embedding dimension & 4 \\
    Index of video frame & 0 \\
    Extension in temporal dim. & Repeat \\
    \midrule\midrule
    \textbf{Temporal Layers}  & \\
    \textit{Architecture}  &  \\
    % Pretrained &\cmark \\
    Transformer depth & 1 \\
    Attention resolutions & 64,32,16 \\
    Head channels & 64\\
    % Input projection & \cmark \\
    Positional encoding &\xmark\\
    % $\dim \alpha$ & 10 \\
    Temporal conv layer num & 4 \\
    Temporal kernel size & 3,1,1 \\
    % \midrule
    % \emph{Concat Conditioning} & \\
    % $\dim c_{S}$  & 4\\
    % Context channels & 128 & 128 & 128 & -   \\
    % Temporal kernel size & 3,1,1 & 3,1,1& 3,1,1 & -\\
    \midrule \midrule
    \textbf{Training}  &  \\
    Parameterization & $\boldsymbol{\varepsilon}$ \\
    \# train steps  & 60K   \\
    Learning rate & $5\times 10^{-4}$  \\
    Batch size per GPU  & 4\\
    \# GPUs  & 8 \\
    GPU-type  & A800-80GB \\
    Sequence length & 16\\
    mask ratio & 0.7 \\
    \midrule\midrule
    \textbf{Diffusion Setup}  &   \\
    Diffusion steps & 1000 \\
    Noise schedule & Linear  \\
    $\beta_{0}$ & 0.00085\\
    $\beta_{T}$ & 0.0120\\
    \midrule\midrule
    \textbf{Sampling Parameters}  &  \\
    Sampler  &  DDIM   \\
    Steps  & 50\\
    $\eta$  & 1.0 \\
    Guidance scale $s_\text{txt}$ & 7.5 \\
    Guidance scale $s_\text{img}$ & 7.5 \\
    \bottomrule
\end{tabular}%
}
\label{table:hyperparameters}
\vspace{-0.4cm}
\end{table}

==> all_subtex/supp_mask_condition.tex <==
% \includegraphics[scale=0.5]{
\begin{figure*}[t]
  \centering
  \begin{tabular}{c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c}
  OF-G  & Output &  SAM-G & Output  \\
  % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
    \includegraphics[width=0.2\linewidth]{images/mask_optical.png} &
    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
    \animategraphics[width=0.2\linewidth]{8}{gif/supp_mask/optical/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
     \includegraphics[width=0.2\linewidth]{images/mask_sam.png}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/supp_mask/sam/frame_}{1}{16}
     % % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
     % \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/OFC_16/frame_}{1}{16}
     % \\
     % \multicolumn{2}{c}{\textit{``walking, driving''}}  & \multicolumn{2}{c}{\textit{``dancing''}} &  &  \\
    \end{tabular}
    
\vspace{-0.7em}
  \caption{\textbf{The comparison between different conditional mask}. \enquote{OF-G} is the mask from optical flow-based motion mask generation and \enquote{SAM-G} .
  % \textit{Best viewed with Acrobat Reader. Click the video to play the animation clips. \textbf{Static frames are provided in supplementary materials.}}
  }
  \vspace{-0.3cm}
\label{fig:mask_different} 
\end{figure*}
% }

==> all_subtex/supp_opm_motion.tex <==
% \includegraphics[scale=0.5]{
\begin{figure*}[t]
  % \centering
  \begin{tabular}{c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c}
  User Click & OFM=4 & OFM=8 & OFM=12 & {OFM=16} \\
  % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
    \includegraphics[width=0.2\linewidth]{images/flag.jpg} &
    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/OFC_4/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/OFC_8/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/FPS_16/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/OFC_16/frame_}{1}{16}
     \\
      \textit{``Fluttering''}  & FPS=4 & FPS=8 & FPS=12 & FPS=16 \\
  % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
    &
    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/FPS_4/frame_}{1}{10}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/FPS_8/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/FPS_12/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion/FPS_16/frame_}{1}{16}\\
  %      User Click & OFM=4 & OFM=8 & OFM=12 & {OFM=16} \\
  % % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
  %   \includegraphics[width=0.2\linewidth]{images/girl_head.jpg} &
  %   % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
  %   \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/OFC_4/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/OFC_8/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/FPS_16/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/OFC_16/frame_}{1}{16}
  %    \\
  %     \textit{``Sad''}  & FPS=4 & FPS=8 & FPS=12 & FPS=16 \\
  % % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
  %   &
  %   % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
  %   \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/FPS_4/frame_}{1}{10}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/FPS_8/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/FPS_12/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/ablation_motion_cry/OFC_8/frame_}{1}{16}\\
    \end{tabular}
    
\vspace{-0.3em}
  \caption{
  \textbf{Comparisons between our optical flow motion magnitude control (OFM) and FPS-based motion magnitude control (FPS)}.
  Our control method can effectively and almost linearly control the motion intensity.
  % Qualitative comparison results between publicly available image-to-video tools and our proposed RegionMaker. 
  {\textit{View with Acrobat Reader to play the animation clips.}}
  % \textbf{Static frames are provided in supplementary materials.}}}
  }
\vspace{-0.3cm}
\label{fig:supp magnitude} 
\end{figure*}
% }

==> all_subtex/supp_quantitive.tex <==
% \includegraphics[scale=0.5]{
\begin{figure*}[!t]
\vspace{-0.3cm}
  % \centering
  \begin{tabular}{c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c@{\hspace{0.1em}}c}
  % User Click & Gen-2~\cite{gen2} & Genmo~\cite{genmo} & Pika Labs~\cite{pikalabs} & {\small Animate-A}~\cite{dai2023animateanything} \\
  % % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
  %   \includegraphics[width=0.2\linewidth]{images/dog.jpg} &
  %   % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
  %   \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_gen/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_genmo/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_pika/frame_}{1}{12}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_aa/frame_}{1}{16}
  %    \\
  %     \textit{``Shake body''}  & SVD~\cite{blattmann2023stable} & Dynamic~\cite{xing2023dynamicrafter} & I2VGen-XL~\cite{pikalabs} & {\small Ours} \\
  % % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
  %   &
  %   % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
  %   \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_svd/frame_}{1}{10}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_dynamicrafter/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/dog_i2v/frame_}{1}{16}&
  %    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
  %    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_dog/ours/frame_}{1}{16}
     User Click & Gen-2~\cite{gen2} & Genmo~\cite{genmo} & Pika Labs~\cite{pikalabs} & {\small Animate-A}~\cite{dai2023animateanything} \\
  % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
    \includegraphics[width=0.2\linewidth]{images/man.jpg} &
    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_gen/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_genmo/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_pika/frame_}{1}{12}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_aa/frame_}{1}{16}
     \\
      \textit{``Tune the head''}  & SVD~\cite{blattmann2023stable} & Dynamic~\cite{xing2023dynamicrafter} & I2VGen-XL~\cite{pikalabs} & {\small Our} \\
  % & {\small I2VGen-XL}~\cite{i2vgenxl} & {\small RegionMaker(ours)}\\
    &
    % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/gen2/011_0.jpg}&
    \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_svd/frame_}{1}{10}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/genmo/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_dynamicrafter/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/pika/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/man_i2v/frame_}{1}{16}&
     % \includegraphics[width=0.14\linewidth]{gif/AZvsOthers/line3/videocrafter/011_0.jpg}&
     \animategraphics[width=0.2\linewidth]{8}{gif/comparison_man/ours/frame_}{1}{16}\\
    \end{tabular}
\vspace{-0.7em}
  \caption{\textbf{Qualitative comparisons between baselines and our approach}.
  %
  We compare with both close-sourced commercial tools including Gen-2~\cite{gen2}, Genmo~\cite{genmo}, and Pika~\cite{pikalabs} and research works including Animate-anything~\cite{dai2023animateanything}, SVD\cite{chai2023stablevideo}, Dynamicrafter\cite{xing2023dynamicrafter}, and I2VGen-XL \cite{i2vgenxl}.
  %
  Please click the video to play the animated clips via \textit{Adobe Acrobat Reader}. 
  %
  \textit{Static frames are provided in supplementary materials}.
  }
  \vspace{-0.5cm}
\label{fig:man Qualitative comparison} 
\end{figure*}
% }
